NPASA: An algorithm for nonlinear programming -- Motivation and Global Convergence

In this paper, we present a two phase method for solving nonlinear programming problems called Nonlinear Polyhedral Active Set Algorithm (NPASA) that has global and local convergence guarantees under reasonable assumptions. The first phase consists of an augmented Lagrangian method to ensure global convergence while the second phase is designed to promote fast local convergence by performing a balanced reduction of two error estimators for nonlinear programs. After presenting error estimators for nonlinear programs and our algorithm NPASA, we establish global convergence properties for NPASA. Local quadratic convergence of NPASA is established in a companion paper.

==> global-phase-one-old.tex <==
\section{Convergence Analysis for Phase One of NPASA} \label{section:npasa-phase-one}
We begin our convergence analysis by providing a detailed discussion and analysis for phase one of NPASA. Motivation for the global step in phase one is to ensure the robustness of the NPASA algorithm. In particular, phase two of NPASA may encounter problems when the linearization of $\bm{h} (\bm{x})$ at the current iterate requires a large perturbation to be feasible resulting in an unsuccessful minimization of $\| \bm{h} (\bm{x}) \|$ in the Constraint Step. In such an instance, phase one serves as a safeguard to move the primal iterates to a new point before attempting phase two again. For phase one we have decided to use augmented Lagrangian techniques. First introduced by Hestenes \cite{Hestenes1969} and Powell \cite{Powell1969} and sometimes referred to as the method of multipliers, augmented Lagrangian methods and their convergence properties have since been well studied \cite{bertsekas1995nonlinear, Luo2008, NandW} and have been successful at solving nonlinear programs in practice using software packages such as ALGENCAN \cite{Andreani2008}, ALGLIB \cite{Bochkanov1999}, LANCELOT \cite{Conn1991, Conn2010}, and MINOS \cite{Murtagh1978}. Hence, the choice of an augmented Lagrangian technique is a suitable safeguard to ensure NPASA will converge to a stationary point in the case that problems arise during the constraint step in phase two.

Consider the minimization problem in the GS algorithm at the $k$th iteration of NPASA given by
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{x} \in \mathbb{R}^{n}} & \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) = f (\bm{x}) + \bm{\bar{\lambda}}_k^{\intercal} \bm{h} (\bm{x}) + q_k \| \bm{h} (\bm{x}) \|^2 \\
\text{s.t.} & \bm{r}(\bm{x}) \leq \bm{0}
\end{array} \label{prob:aug-lag-mod}
\end{align}
where $\bm{r} (\bm{x}) = \bm{A} \bm{x} - \bm{b}$ is the linear function from problem (\ref{prob:main-nlp}) and $\bm{\bar{\lambda}}_k = Proj_{[-\bar{\lambda}, \bar{\lambda}]} (\bm{\lambda}_k)$ is known. Now suppose that $\bm{x}_{k+1}$ is a stationary point for problem (\ref{prob:aug-lag-mod}). Then by the KKT conditions there exists a $\bm{\mu}_{k+1} \geq \bm{0}$ such that
\begin{align}
\bm{0} 
&= \nabla_x \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) + \bm{\mu}_{k+1}^{\intercal} \bm{A} \\
&= \nabla f (\bm{x}_{k+1}) + (\bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}_{k+1}))^{\intercal} \nabla \bm{h} (\bm{x}_{k+1}) + \bm{\mu}_{k+1}^{\intercal} \bm{A} \\
&= \nabla \mathcal{L} (\bm{x}_{k+1}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}_{k+1}), \bm{\mu}_{k+1})
\end{align}
and $\bm{\mu}_{k+1}^{\intercal} \bm{r} (\bm{x}_{k+1}) = 0$. Taking $\bm{\lambda}_{k+1} = \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}_{k+1})$, it now follows from the definition of $E_{m,0}$ that
\begin{align}
E_{m,0} (\bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1}) = 0.
\end{align}
Note that we can solve problem (\ref{prob:aug-lag-mod}) using the algorithm PASA \cite{HagerActive}. If PASA is used to solve problem (\ref{prob:aug-lag-mod}) and it converges to a stationary point $\bm{x}_{k+1}$ then we have that the multiplier error is equal to zero at $(\bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1})$, where $\bm{\mu}_{k+1}$ is some vector that we do not explicitly know. The global error estimator used for stopping criterion in PASA at a point $\bm{x} \in \Omega$ is given by $E_{\scaleto{PASA}{4pt}} (\bm{x}) = \| \bm{y} (\bm{x},1) - \bm{x} \|$ where $\bm{y} (\bm{x},\alpha)$ is defined to be the minimizer for the problem
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{y}} & \displaystyle \frac{1}{2} \| \bm{x} - \alpha \bm{g} (\bm{x}) - \bm{y} \|^2 \\
\text{s.t.} & \bm{r}(\bm{y}) \leq \bm{0}
\end{array} \label{prob:pasa-error}
\end{align} 
for $\alpha > 0$ and where $\bm{g} (\bm{x})$ is the transpose of the gradient of the cost function in the polyhedral constrained problem being solved by PASA. Note that in our case we have 
\begin{align}
\bm{g} (\bm{x})^{\intercal} 
&= \nabla_x \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) 
= \nabla f (\bm{x}) + \bm{\bar{\lambda}}_k^{\intercal} \nabla \bm{h} (\bm{x}) + 2 q_k \bm{h} (\bm{x})^{\intercal} \nabla \bm{h} (\bm{x}) \label{eq:aug-lag-mod.0.0}
\end{align} 
but we will continue to write $\bm{g} (\bm{x})$ for simplicity. When an iterate $\bm{x} \in \Omega$ of PASA results in $E_{\scaleto{PASA}{4pt}} (\bm{x})$ being sufficiently small, where the tolerance is set by the user, then PASA terminates. Now fix $\bm{x} \in \Omega$ and consider problem (\ref{prob:pasa-error}). By the KKT conditions, there exists a vector $\bm{\mu}(\bm{x},\alpha)$ such that
\begin{enumerate}
\item[(\ref{prob:pasa-error}.1)] Gradient of Lagrangian equals zero: $(\bm{y}(\bm{x},\alpha) - \bm{x})^{\intercal} + \alpha \bm{g} (\bm{x})^{\intercal} + \bm{\mu}(\bm{x}, \alpha)^{\intercal} \bm{A} = \bm{0}$
\item[(\ref{prob:pasa-error}.2)] Satisfies inequality constraints: $\bm{r}(\bm{y}(\bm{x},\alpha)) \leq \bm{0}$
\item[(\ref{prob:pasa-error}.3)] Nonnegativity of inequality multipliers: $\bm{\mu} (\bm{x},\alpha) \geq \bm{0}$
\item[(\ref{prob:pasa-error}.4)] Complimentary slackness: $\bm{\mu} (\bm{x},\alpha)^{\intercal} \bm{r}(\bm{y}(\bm{x},\alpha)) = 0$.
\end{enumerate}
Our goal is to use the KKT conditions (\ref{prob:pasa-error}.1) -- (\ref{prob:pasa-error}.4) for problem (\ref{prob:pasa-error}) to derive a formula for the multiplier error of our original problem, $E_{m,0}$, in terms of the current iterate of PASA. Then we will show that we can bound this expression for $E_{m,0}$ in terms of the global error estimator of PASA. This is summarized in the following result.
\begin{lemma} \label{lem:Em0-Epasa-comparison}
Suppose $\bm{x} \in \Omega$. Then for each $\alpha > 0$ there exists an inequality multiplier $\bm{\mu} (\bm{x},\alpha)$ such that 
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x},\alpha)/\alpha) 
&= - \bm{g}(\bm{x})^{\intercal} (\bm{y}(\bm{x},\alpha) - \bm{x}) + \left(\frac{1}{\alpha^2} - \frac{1}{\alpha} \right) \| \bm{y}(\bm{x},\alpha) - \bm{x} \|^2. \label{eq:aug-lag-mod.4}
\end{align}
In particular, if $\alpha = 1$ then
\begin{align}
E_{\scaleto{PASA}{4pt}} (\bm{x})^2 
&\leq E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) 
\leq \| \nabla_x \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) \| E_{\scaleto{PASA}{4pt}} (\bm{x}) \label{eq:aug-lag-mod.5}
\end{align}
and $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) = 0$ if and only if $\bm{x}$ is a stationary point for problem (\ref{prob:aug-lag-mod}).
\end{lemma}
\begin{proof}
Let $\bm{x} \in \Omega$. By recalling that the multiplier error estimator $E_{m,0}$ for problem (\ref{prob:main-nlp}) is given by $E_{m,0} (\bm{x}, \bm{\lambda}, \bm{\mu}) = \| \nabla f (\bm{x}) + \bm{\lambda}^{\intercal} \nabla \bm{h} (\bm{x}) + \bm{\mu}^{\intercal} \bm{A} \|^2 - \bm{\mu}^{\intercal} \bm{r} (\bm{x})$, it follows that 
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu}) 
&= \| \bm{g} (\bm{x})^{\intercal} + \bm{\mu}^{\intercal} \bm{A} \|^2 - \bm{\mu}^{\intercal} \bm{r} (\bm{x}). \label{eq:aug-lag-mod.0}
\end{align} 
With this in mind, we now proceed as follows. First, from (\ref{prob:pasa-error}.1) we have that
\begin{align}
\bm{g} (\bm{x})^{\intercal} + \frac{1}{\alpha} \bm{\mu} (\bm{x},\alpha)^{\intercal} \bm{A} = \frac{1}{\alpha}(\bm{x} - \bm{y}(\bm{x},\alpha))^{\intercal}
\end{align}
Now taking the norm of both sides and squaring yields
\begin{align}
\left\| \bm{g} (\bm{x})^{\intercal} + \frac{1}{\alpha} \bm{\mu} (\bm{x},\alpha)^{\intercal} \bm{A} \right\|^2 = \frac{1}{\alpha^2} \| \bm{y}(\bm{x},\alpha) - \bm{x} \|^2. \label{eq:aug-lag-mod.1}
\end{align}
Additionally, right multiplying both sides of (\ref{prob:pasa-error}.1) by $\frac{1}{\alpha} (\bm{y}(\bm{x},\alpha) - \bm{x})$ and using (\ref{prob:pasa-error}.4) yields
\begin{align}
- \frac{1}{\alpha} \bm{\mu}(\bm{x},\alpha)^{\intercal} \bm{r}(\bm{x}) = - \frac{1}{\alpha} \| \bm{y}(\bm{x},\alpha) - \bm{x} \|^2 - \bm{g}(\bm{x})^{\intercal} (\bm{y}(\bm{x},\alpha) - \bm{x}). \label{eq:aug-lag-mod.2}
\end{align}
%Note that as $\bm{x} \in \Omega$ we have that $-\bm{\mu}(\bm{x})^{\intercal} \bm{A} \bm{x} \geq 0$ which implies that $\nabla_x \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y}(\bm{x}) - \bm{x}) \leq \bm{0}$. 
Combining (\ref{eq:aug-lag-mod.0}), (\ref{eq:aug-lag-mod.1}), and (\ref{eq:aug-lag-mod.2}) yields (\ref{eq:aug-lag-mod.4}). 

Next, note that from property P6 in Proposition 2.1 of \cite{Hager2006} we have that for all $\bm{x} \in \Omega$
\begin{align}
- \bm{g} (\bm{x})^{\intercal} (\bm{y}(\bm{x},\alpha) - \bm{x}) \geq \frac{1}{\alpha} \| \bm{y}(\bm{x},\alpha) - \bm{x} \|^2.
\end{align}
Combining this fact with (\ref{eq:aug-lag-mod.4}) yields a lower bound for the multiplier error
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x},\alpha)/\alpha) 
\geq \frac{1}{\alpha^2} \| \bm{y}(\bm{x},\alpha) - \bm{x} \|^2. \label{eq:aug-lag-mod.4.1}
\end{align}
In particular, by taking $\alpha = 1$ in (\ref{eq:aug-lag-mod.4}) and recalling (\ref{eq:aug-lag-mod.0.0}) we have
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) 
= - \nabla_x \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y}(\bm{x},1) - \bm{x}). \label{eq:aug-lag-mod.4.2}
\end{align}
Now combining (\ref{eq:aug-lag-mod.4.1}) and (\ref{eq:aug-lag-mod.4.2}) with the definition of $E_{\scaleto{PASA}{4pt}} (\bm{x})$ and Cauchy-Schwarz yields (\ref{eq:aug-lag-mod.5}). 

Lastly, as $E_{\scaleto{PASA}{4pt}} (\bm{x}) = 0$ if and only if $\bm{x}$ is a stationary point \cite{HagerActive}, we conclude from (\ref{eq:aug-lag-mod.5}) that $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) = 0$ if and only if $\bm{x}$ is a stationary point. 
\end{proof}

Hence, in (\ref{eq:aug-lag-mod.4}) we have derived a closed form expression for the multiplier error estimator for the general nonlinear program in terms of the current iterate of PASA and a known KKT equality multiplier. Additionally, in (\ref{eq:aug-lag-mod.5}) upper and lower bounds for the multiplier error estimator for the general nonlinear program were derived in terms of the global error estimator used by PASA. Thus, we can compute and bound the value of the multiplier error estimator $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}(\bm{x}_k,\alpha))$ by using information already computed by PASA without requiring the inequality multiplier vector $\bm{\mu}(\bm{x}_k,\alpha)$. We now provide the following result which will be useful to note for practical implementations of this approach for augmented Lagrangian problems. The result follows immediately from (\ref{eq:aug-lag-mod.5}) and the definition of the dot product.

\begin{theorem} \label{thm:pasa-aug-lag-conv}
Suppose that PASA with $\varepsilon = 0$ generates an infinite sequence of iterates $\{ \bm{u}_i \}_{i=1}^{\infty}$ such that
\begin{align}
\| \nabla_x \mathcal{L}_{q_k} (\bm{u}_i, \bm{\bar{\lambda}}_k) \| \cos (\theta_i) \leq C, \label{result:pasa-aug-lag-conv.1}
\end{align}
for all $i$, where $C$ is some constant and $\theta_i$ is the angle between the vectors $\bm{u}_i - \bm{y}(\bm{u}_i,1)$ and $\mathcal{L}_{q_k} (\bm{u}_i, \bm{\bar{\lambda}}_k)$. Then $\displaystyle \liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) = 0$ if and only if $\displaystyle \liminf_{i \to \infty} E_{\scaleto{PASA}{4pt}} (\bm{u}_i) = 0$.
\end{theorem}
\iffalse
\begin{proof}
By definition of the dot product, it follows from (\ref{eq:aug-lag-mod.4.2}) and our hypothesis that
\begin{align*}
E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{u}_i,1)) 
&= \| \nabla_x \mathcal{L}_{q_k} (\bm{u}_i, \bm{\bar{\lambda}}_k)\| \| \bm{y}(\bm{u}_i,1) - \bm{u}_i \| \cos (\theta_i) \\
&= \| \nabla_x \mathcal{L}_{q_k} (\bm{u}_i, \bm{\bar{\lambda}}_k)\| \cos (\theta_i) E_{\scaleto{PASA}{4pt}} (\bm{u}_i) \\
&\leq C E_{\scaleto{PASA}{4pt}} (\bm{u}_i).
\end{align*}
Combining this with the lower bound on $E_{m,0}$ we have that
\begin{align*}
E_{\scaleto{PASA}{4pt}} (\bm{u}_i)^2 
\leq E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) 
\leq C E_{\scaleto{PASA}{4pt}} (\bm{u}_i)
\end{align*}
which concludes the proof.
\end{proof}
\fi

Before providing a convergence result for this approach to phase one of NPASA, we consider how convergence of PASA for the subproblem in phase one relates to the multiplier error estimator of the original nonlinear program, (\ref{prob:main-nlp}). In particular, since our branching criterion in phase one of NPASA is given by $E_{m,1} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k) \leq \theta E_c (\bm{x}_k)$ and $E_{m,1} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k) \leq E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k)$, we would like some conditions under which PASA converges to a point $\bm{x}_k$ at which $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k) \approx 0$. The following result is a natural first step as it is a global convergence result for the multiplier error based on the global convergence result for PASA in \cite{Hager2016} that only requires one assumption in addition to those already imposed in \cite{Hager2016} to establish global convergence of PASA. First, we need to set up the assumptions that are used in this result as they are based on details of the algorithm PASA \cite{HagerActive}. Given $\bm{u} \in \mathbb{R}^n$, $\bm{\nu} \in \mathbb{R}^s$, and $q$ we define the level set $\mathcal{S}(\bm{u}, \bm{\nu}, q) := \{ \bm{x} \in \Omega : \mathcal{L}_q (\bm{x}, \bm{\nu}) \leq \mathcal{L}_q (\bm{u}, \bm{\nu}) \}$. Additionally, we let the set $\mathcal{D}(\bm{u}, \bm{\nu}, q)$ denote the search directions generated by phase one of the algorithm PASA \cite{HagerActive} when solving the problem 
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{x}} & \displaystyle \mathcal{L}_q (\bm{x}, \bm{\nu}) \\
\text{s.t.} & \bm{x} \in \Omega
\end{array} \label{prob:aug-lag-intro}
\end{align}
starting at the initial guess $\bm{x} = \bm{u}$. Note that the definition of the search directions generated in phase one of PASA can be found in Algorithm 1 in Section 2 of \cite{HagerActive}. We are now ready to state the assumptions:
\begin{enumerate}
\item[(G1)] Given $\bm{u} \in \mathbb{R}^n$ and $\bm{\nu} \in \mathbb{R}^s$, $\mathcal{L}_q (\bm{x}, \bm{\nu})$ is bounded from below on the level set $\mathcal{S} (\bm{u}, \bm{\nu})$ and $d_{\max} = \sup_{\bm{d} \in \mathcal{D}(\bm{u}, \bm{\nu}, q)} \| \bm{d} \| < \infty$
\item[(G2)] Given $\bm{u} \in \mathbb{R}^n$ and $\bm{\nu} \in \mathbb{R}^s$, if $\overline{\mathcal{S}}(\bm{u}, \bm{\nu})$ is the collection of $\bm{x} \in \Omega$ whose distance to $\mathcal{S}(\bm{u}, \bm{\nu})$ is at most $d_{\max}$, then $\nabla_x \mathcal{L}_q (\bm{x}, \bm{\nu})$ is Lipschitz continuous on $\overline{\mathcal{S}}(\bm{u}, \bm{\nu})$.
\end{enumerate}

\begin{theorem} \label{thm:pasa-aug-lag}
Given $\bm{u}_0 \in \mathbb{R}^n$, $\bm{\bar{\lambda}}_k$, and $q_k$ suppose that (G1) and (G2) hold at $(\bm{u}_0, \bm{\bar{\lambda}}_k, q_k)$. Then PASA with $\varepsilon = 0$ either terminates in a finite number of iterations to a stationary point, $\bm{u}^*$, at which
\begin{align*}
E_{m,0} (\bm{u}^*, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}^*), \bm{\mu} (\bm{u}^*,1)) = 0
\end{align*}
or PASA generates a sequence of points $\{ \bm{u}_i \}_{i=1}^{\infty}$ with the property that 
\begin{align}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) = 0
\end{align}
if, in addition to (G1) and (G2), (\ref{result:pasa-aug-lag-conv.1}) holds for the sequence $\{ \bm{u}_i \}_{i=1}^{\infty}$.
\end{theorem}
\begin{proof}
As the hypotheses of Theorem 3.2 in \cite{Hager2016} are satisfied for problem (\ref{prob:aug-lag-mod}), we have that either PASA converges to a stationary point $\bm{u}^*$, at which $E_{\scaleto{PASA}{4pt}} (\bm{u}^*) = 0$ or $\liminf_{i \to \infty} E_{\scaleto{PASA}{4pt}} (\bm{u}_i) = 0$. The result now follows from Theorem~\ref{thm:pasa-aug-lag-conv}.
% (Incorrect argument that thgouht we didn't need boundedness assumption)
\iffalse
Next, note that the set $\bar{\mathcal{L}}$ described in assumption A2 used as a hypothesis for Theorem 3.2 in \cite{Hager2016} is a closed and bounded set. As $\nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k)$ is continuous we have that $\| \nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k) \|$ attains its maximum value on $\bar{\mathcal{L}}$. Finally, as $\bm{u}_i \in \bar{\mathcal{L}}$ for all $i$, we have that the sequence $\{ \| \nabla \mathcal{L}_q (\bm{u}_i, \bm{\bar{\lambda}}_k) \| \}_{i = 0}^{\infty}$ is uniformly bounded. Now using inequality (\ref{eq:aug-lag-mod.5}) together with (\ref{eq:thm3.2-pasa.1}) and (\ref{eq:thm3.2-pasa.2}) concludes the proof.
\fi
%
\end{proof}

Next, we provide a result that holds when PASA generates an infinite sequence of iterates that converge to a stationary point but does not require as many assumptions as the global convergence result.

\begin{theorem} \label{thm:pasa-aug-lag-degenerate}
If PASA with $\varepsilon = 0$ generates an infinite sequence of iterates $\{ \bm{u}_i \}_{i=1}^{\infty}$ that converge to a stationary point $\bm{u}^*$ then
\begin{align}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i)) = 0. \label{result:aug-lag-degenerate.1}
\end{align}
\end{theorem}
\begin{proof}
As $\bm{u}^*$ is a stationary point, we have that $\bm{y} (\bm{u}^*) = \bm{u}^*$. So by (\ref{prob:pasa-error}.1) - (\ref{prob:pasa-error}.4) we have that $\bm{\mu}(\bm{u}^*) \geq \bm{0}$ satisfies $\nabla \mathcal{L}_{q_k} (\bm{u}^*, \bm{\bar{\lambda}}_k) + \bm{\mu}(\bm{u}^*)^{\intercal} \bm{A} = \bm{0}$ and $\bm{\mu}(\bm{u}^*)^{\intercal} \bm{A} \bm{u}^* = 0$. Hence, it follows that $E_{m,0} (\bm{u}^*, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}^*), \bm{\mu} (\bm{u}^*)) = 0$. As $\bm{u}_i \to \bm{u}^*$ and $\bm{\mu} (\bm{u}_i) \to \bm{\mu}(\bm{u}^*)$ when $i \to \infty$ and $E_{m,0}$ is continuous, the result in (\ref{result:aug-lag-degenerate.1}) follows.
\end{proof}

In addition to the global convergence result in Theorem~\ref{thm:pasa-aug-lag}, we would like to determine if we can establish an alternative bound on the directional derivative appearing in the formula for the multiplier error (\ref{eq:aug-lag-mod.4.2}) under a different set of assumptions. This is of interest as the upper bound in (\ref{eq:aug-lag-mod.5}) may be problematic if, say, in practice the term $\| \nabla_x \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) \|$ grows larger as $\bm{x}$ gets closer to a stationary point. We now consider the following. First, note that the local error estimator used by PASA for this problem is defined by $e_{\scaleto{PASA}{4pt}} (\bm{x}) = \| \bm{g}^{\mathcal{A}} (\bm{x}) \|$, where 
\begin{align}
\bm{g}^{\mathcal{A}} (\bm{x}) = \arg\min \{ \| \bm{z} - \bm{g} (\bm{x}) \| : \bm{z} \in \mathbb{R}^n \ \text{and} \ \bm{A}_{\mathcal{A} (\bm{x})} \bm{z} = \bm{0} \},
\end{align}
where $\mathcal{A} (\bm{x}) = \{ i : (\bm{A} \bm{x})_i = 0 \}$. By this definition, we can decompose $\bm{g} (\bm{x})$ as
\begin{align}
\bm{g} (\bm{x}) = \bm{g}^{\mathcal{A}} (\bm{x}) + \bm{g}^{\mathcal{A}^{\perp}} (\bm{x})
\end{align}
where $\bm{g}^{\mathcal{A}^{\perp}} (\bm{x}) \perp \mathcal{N} \left( A_{\mathcal{A} (\bm{x})} \right)$. Now using the formula in (\ref{eq:aug-lag-mod.4.2}) yields
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},1)) 
&= \bm{g} (\bm{x})^{\intercal} (\bm{x} - \bm{y} (\bm{x},1)) \\
&= \left( \bm{g}^{\mathcal{A}} (\bm{x}) + \bm{g}^{\mathcal{A}^{\perp}} (\bm{x}) \right)^{\intercal} (\bm{x} - \bm{y} (\bm{x},1)) \\ 
&= \bm{g}^{\mathcal{A}} (\bm{x})^{\intercal} (\bm{x} - \bm{y} (\bm{x},1)) + \bm{g}^{\mathcal{A}^{\perp}} (\bm{x})^{\intercal} (\bm{x} - \bm{y} (\bm{x},1)). \label{eq:aug-lag-mod.6}
\end{align}
So if at some point $\bm{x} \in \Omega$ we have that $(\bm{x} - \bm{y} (\bm{x},1) ) \in \mathcal{N} (\bm{A}_{\mathcal{A}(\bm{x})})$ then it follows from (\ref{eq:aug-lag-mod.6}) that
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) 
= \nabla_x \mathcal{L}_{q_k}^{\mathcal{A}} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{x} - \bm{y}(\bm{x},1)) \label{eq:aug-lag-mod.7}
\end{align}
and in such a case Cauchy-Schwarz yields
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) 
\leq e_{\scaleto{PASA}{4pt}} (\bm{x}) E_{\scaleto{PASA}{4pt}} (\bm{x}). \label{eq:aug-lag-mod.8}
\end{align}
In the case that PASA converges to a nondegenerate stationary point, we have the following result.
\begin{theorem} \label{thm:pasa-aug-lag-nondegenerate}
If PASA with $\varepsilon = 0$ generates an infinite sequence of iterates $\{ \bm{u}_i \}_{i=1}^{\infty}$ that converge to a nondegenerate stationary point $\bm{u}^*$, then there exists an integer $M$ such that 
\begin{align}
E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) 
\leq e_{\scaleto{PASA}{4pt}} (\bm{u}_i) E_{\scaleto{PASA}{4pt}} (\bm{u}_i), \label{result:aug-lag-nondegenerate.1}
\end{align}
for all $i \geq M$. 
% (Not necessary since better result established)
\iffalse
, and we have that
\begin{align}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) = 0. \label{result:aug-lag-nondegenerate.2}
\end{align}
\fi
%
\end{theorem}
\begin{proof}
By equations (5.3) and (5.4) in Theorem 5.1 of \cite{Hager2016}, there exists an integer $M$ such that 
\begin{align*}
\mathcal{A} (\bm{u}_i) \subseteq \mathcal{A} (\bm{y}(\bm{u}_i,1))
\end{align*}
for all $i \geq M$. Hence, for all $i \geq M$ we have that $(\bm{u}_i - \bm{y} (\bm{u}_i,1)) \in \mathcal{N}(\bm{A}_{\mathcal{A}(\bm{u}_i)})$ since
\begin{align*}
\bm{A}_{\mathcal{A}(\bm{u}_i)} (\bm{u}_i - \bm{y} (\bm{u}_i,1))
= \bm{b}_{\mathcal{A}(\bm{u}_i)} - \bm{b}_{\mathcal{A}(\bm{u}_i)}
= \bm{0}.
\end{align*}
By (\ref{eq:aug-lag-mod.7}), we now have
\begin{align*}
E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) 
&= \nabla \mathcal{L}_{q_k}^{\mathcal{A}} (\bm{u}_i, \bm{\bar{\lambda}}_k) (\bm{u}_i - \bm{y} (\bm{u}_i,1)),
\end{align*}
for all $i \geq M$. Now applying Cauchy-Schwarz to the right hand side of this equation and recalling the definition of $e_{\scaleto{PASA}{4pt}} (\cdot)$ and $E_{\scaleto{PASA}{4pt}} (\cdot)$ yields (\ref{result:aug-lag-nondegenerate.1}), for all $i \geq M$.
% (Proof for unnecessary result)
\iffalse
As $\bm{u}_i \to \bm{u}^*$ and $E_{\scaleto{PASA}{4pt}} (\bm{u}^*) = 0$, we have that there exists a constant $C$ such that
\begin{align}
E_{\scaleto{PASA}{4pt}} (\bm{u}_i) \leq C, \label{eq:aug-lag-nondegenerate.1}
\end{align}
for $i \geq M$. By Theorem 5.1 in \cite{Hager2016}, only phase two of PASA is executed within a finite number of iterations so we focus on the LCO method used in phase two of PASA. From condition F2 for phase two of PASA in \cite{Hager2016} and the fact that $\bm{u}_i$ is finite dimensional it follows that $\mathcal{A} (\bm{u}_i)$ is fixed for $i$ sufficiently large. Hence, by condition F3 for phase two of PASA in \cite{Hager2016} we have that
\begin{align}
\liminf_{i \to \infty} e_{\scaleto{PASA}{4pt}} (\bm{u}_i) = 0. \label{eq:aug-lag-nondegenerate.2}
\end{align}
Now (\ref{eq:aug-lag-nondegenerate.1}) and (\ref{eq:aug-lag-nondegenerate.2}) together with (\ref{result:aug-lag-nondegenerate.1}) yields (\ref{result:aug-lag-nondegenerate.2}).
\fi
%
% (I believe the following version is not always true since e(x) may not be bounded)
\iffalse
As $\bm{u}_i \to \bm{u}^*$ and 
\begin{align*}
E_{\scaleto{PASA}{4pt}} (\bm{u}^*) = 0, 
\end{align*}
it now follows from (\ref{eq:aug-lag-nondegenerate.1}) that
\begin{align*}
\liminf_{i \to \infty} E_m (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i)) \leq \left( \liminf_{i \to \infty} e_{\scaleto{PASA}{4pt}} (\bm{u}_i) \right) \left( \lim_{i \to \infty} E_{\scaleto{PASA}{4pt}} (\bm{u}_i) \right) = 0
\end{align*}
which concludes the proof.
\fi
%
\end{proof}

If we include second order assumptions then we can obtain an upper bound for the multiplier error in degenerate problems. This result follows from some standard analysis and an application of Lemma 6.4 from \cite{Hager2016}.
\begin{theorem} \label{thm:pasa-aug-lag-degenerate2}
Suppose that $\mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k)$ is twice continuously differentiable in a neighborhood of a local minimizer $\bm{x}^*$ where the active constraint gradients are linearly independent and the strong second-order sufficient optimality conditions hold. Then there exists a $\rho > 0$ such that for all $\bm{x} \in \mathcal{B}_{\rho} (\bm{x}^*)$ 
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x})) 
= O \left( E_{\scaleto{PASA}{4pt}} (\bm{x}) \right), \label{result:aug-lag-degenerate2.1}
\end{align}
where $\kappa$ is a Lipschitz constant for $\nabla_x \mathcal{L}_{q_k} (\bm{x}, \bm{\lambda})$ on $\mathcal{B}_{\rho} (\bm{x}^*)$.
\end{theorem}
\begin{proof}
Using the formula in (\ref{eq:aug-lag-mod.4}) we have that
\begin{align*}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x}))
&= \nabla \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{x} - \bm{y}(\bm{x})) \\
&= \left( \nabla \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) - \nabla \mathcal{L}_{q_k} (\bm{x}^*, \bm{\bar{\lambda}}_k) \right) (\bm{x} - \bm{y}(\bm{x})) + \nabla \mathcal{L}_{q_k} (\bm{x}^*, \bm{\bar{\lambda}}_k) (\bm{x} - \bm{y}(\bm{x}))
\end{align*}
which yields
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x}))
&\leq \kappa \| \bm{x} - \bm{x}^* \| E_{\scaleto{PASA}{4pt}} (\bm{x}) + \| \nabla_x \mathcal{L}_{q_k} (\bm{x}^*, \bm{\bar{\lambda}}_k) \| E_{\scaleto{PASA}{4pt}} (\bm{x})
\end{align}
when applying Cauchy-Schwarz, the triangle inequality, and the Lipschitz continuity of $\nabla \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k)$. Finally, applying Lemma 6.4 from \cite{Hager2016} yields
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x}))
&\leq \kappa \sqrt{1 + \left( \frac{2 (1 + \kappa) ( 3 + \kappa)}{\sigma} \right)} E_{\scaleto{PASA}{4pt}} (\bm{x})^2 \\
&\hspace{3.4mm}+ \| \nabla_x \mathcal{L}_{q_k} (\bm{x}^*, \bm{\bar{\lambda}}_k) \| E_{\scaleto{PASA}{4pt}} (\bm{x}), \nonumber
\end{align}
which concludes the proof.
\end{proof}

With Theorems~\ref{thm:pasa-aug-lag} -- \ref{thm:pasa-aug-lag-degenerate2} established, it seems that this is a suitable approach for solving the subproblem in phase one of NPASA that allows us to still compute the multiplier error estimator. We now provide a result on convergence of phase one of NPASA when using this approach for solving each subproblem.

\begin{theorem} \label{thm:pasa-aug-lag-global-conv}
Suppose that $\Omega$ is compact and that $f, \bm{h} \in \mathcal{C}^1 (\Omega)$. Suppose that the following are satisfied:
\begin{enumerate}
\item $\{ \bm{x}_k \}_{k=0}^{\infty}$ is a sequence with $\bm{x}_k \in \Omega$ and $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}(\bm{x}_k,1)) \leq \theta E_c (\bm{x}_k)$, for all $k \geq 0$
\item $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ is updated using the formula for $\bm{\lambda}'$ in GS algorithm, Algorithm~\ref{alg:gs}
\item $\{ q_k \}_{k=0}^{\infty}$ is a sequence of real numbers such that $q_k \to \infty$ as $k \to \infty$.
\end{enumerate}
Then any subsequence of $\{ \bm{x}_k \}_{k=0}^{\infty}$ with limit point $\bm{x}^*$ such that assumption (\textbf{LI}) holds at $\bm{x}^*$ satisfies $E_1 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu}(\bm{x}^*,1)) = E_0 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu}(\bm{x}^*,1)) = 0$, where $\bm{\lambda}^*$ is the limit of the corresponding subsequence for $\{ \bm{\lambda}_k \}$.
\end{theorem}
\begin{proof}
Let $\{ \bm{x}_k \}_{k=0}^{\infty}$ be a subsequence with limit point $\bm{x}^*$ and let $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu} (\bm{x}_k,1) \}_{k=0}^{\infty}$ be corresponding subsequences of multipliers. First, we show that $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu} (\bm{x}_k,1) \}_{k=0}^{\infty}$ are uniformly bounded for $k$ sufficiently large. Rearranging the terms in equation (\ref{prob:pasa-error}.1) with $\alpha = 1$ we have that 
\begin{align}
\begin{bmatrix}
\nabla \bm{h} (\bm{x}_k)^{\intercal} \ \vert \ \bm{A}^{\intercal}
\end{bmatrix} \begin{bmatrix}
\bm{\lambda}_k \\
\bm{\mu} (\bm{x}_k,1)
\end{bmatrix}
= \bm{x}_k - \bm{y}(\bm{x}_k,1) - \nabla f (\bm{x}_k)^{\intercal}
\end{align}
By our hypothesis that (\textbf{LI}) holds at $\bm{x}^*$, there exists a $N$ such that the matrix $\begin{bmatrix} \nabla \bm{h} (\bm{x}_k)^{\intercal} \ \vert \ \bm{A}^{\intercal} \end{bmatrix}$ is of full column rank, for all $k \geq N$. Hence, there exists a constant $M$ such that
\begin{align}
\left\| \begin{bmatrix}
\bm{\lambda}_k \\
\bm{\mu} (\bm{x}_k,1)
\end{bmatrix} \right\|
\leq M \| \bm{x}_k - \bm{y}(\bm{x}_k,1) - \nabla f (\bm{x}_k)^{\intercal} \|, \label{eq:phase-one-convergence.1}
\end{align}
for $k$ sufficiently large. From property P6 in Proposition 2.1 of \cite{Hager2006} we have that
\begin{align}
\| \bm{x}_k - \bm{y}(\bm{x}_k,1) \|^2 \leq \nabla_x \mathcal{L}_{q} (\bm{x}_k, \bm{\bar{\lambda}}_{k-1})^{\intercal} (\bm{x}_k - \bm{y}(\bm{x}_k,1)).
\end{align}
Hence, using the hypothesis that $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}(\bm{x}_k,1)) \leq \theta E_c (\bm{x}_k)$ together with (\ref{eq:aug-lag-mod.4}) it follows that
\begin{align}
\| \bm{x}_k - \bm{y}(\bm{x}_k,1) \|^2 \leq E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1)) 
\leq E_c (\bm{x}_k).
\end{align}
As $E_c (\bm{x}_k) = \| \bm{h} (\bm{x}_k) \|^2$, the inequality in (\ref{eq:phase-one-convergence.1}) now yields
\begin{align}
\left\| \begin{bmatrix}
\bm{\lambda}_k \\
\bm{\mu} (\bm{x}_k,1)
\end{bmatrix} \right\|
\leq M \left( \| \bm{h} (\bm{x}_k) \| + \| \nabla f (\bm{x}_k) \| \right), \label{eq:phase-one-convergence.2}
\end{align}
for $k$ sufficiently large. As $f, \bm{h} \in \mathcal{C}^1$, it follows from (\ref{eq:phase-one-convergence.2}) that the sequences $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu}(\bm{x}_k,1) \}_{k=0}^{\infty}$ are uniformly bounded for $k$ sufficiently large. As the sequence $\{ \bm{\bar{\lambda}}_k \}_{k=0}^{\infty}$ is uniformly bounded by construction, there exists a constant $\Lambda$ such that $\| \bm{\lambda}_{k} - \bm{\bar{\lambda}}_{k-1} \| \leq \Lambda$ for all $k$ sufficiently large. Now using the update formula $\bm{\lambda}_{k} = \bm{\bar{\lambda}}_{k-1} + 2 q_k \bm{h} (\bm{x}_{k})$, we have that
\begin{align}
\| \bm{h} (\bm{x}_{k}) \| 
= \frac{\| \bm{\lambda}_{k} - \bm{\bar{\lambda}}_{k-1} \|}{2 q_k} 
\leq \frac{\Lambda}{2 q_k}, \label{eq:phase-one-convergence.3}
\end{align}
for all $k$ sufficiently large. So (\ref{eq:phase-one-convergence.3}) together with the hypothesis that $q_k \to \infty$ as $k \to \infty$, yields that
\begin{align}
\lim_{k \to \infty} E_c (\bm{x}_{k}) = \lim_{k \to \infty} \| \bm{h} (\bm{x}_{k}) \|^2 \leq \lim_{k \to \infty} \frac{\Lambda^2}{4 q_k^2} = 0.
\end{align}
As $E_0 (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1))^2 = E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1)) + E_c (\bm{x}_k)$ and $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1)) \leq \theta E_c (\bm{x}_k)$ for all $k$ by hypothesis, it now follows that $E_0 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu} (\bm{x}^*,1)) = 0$. Lastly, from Lemma~\ref{lem:E0-E1-relationship} it follows that $E_1 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu} (\bm{x}^*,1)) = 0$ which concludes the proof.
\end{proof}

%
\iffalse
\begin{theorem}
Suppose that the following are satisfied
\begin{enumerate}
\item $\{ \bm{x}_k \}_{k=0}^{\infty}$ is a sequence with $\bm{x}_k \in \Omega$ and $E_m (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}(\bm{x}_k)) \leq \theta E_c (\bm{x}_k)$, for all $k \geq 0$
\item There exists a scalar $\eta < \infty$ such that $\sup_{k \geq 0} E_{\scaleto{PASA}{4pt}} (\bm{x}_k) \leq \eta$
\item $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ is updated using the formula described after Algorithm~\ref{alg:npasa}
\item $\{ q_k \}_{k=0}^{\infty}$ is a sequence of reals numbers such that $q_k \to \infty $ as $k \to \infty$.
\end{enumerate}
Then any subsequence of $\{ \bm{x}_k \}_{k=0}^{\infty}$ with limit point $\bm{x}^*$ such that $\nabla \bm{h} (\bm{x}^*)$ and $\nabla \bm{r} (\bm{x}^*)$ are of full rank satisfies $E_0 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu}(\bm{x}^*)) = 0$, where $\bm{\lambda}^*$ is the limit of the corresponding subsequence for $\{ \bm{\lambda}_k \}$.
\end{theorem}
\begin{proof}
Let $\{ \bm{x}_k \}_{k=0}^{\infty}$ be a subsequence with limit point $\bm{x}^*$ and let $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu} (\bm{x}_k,1) \}_{k=0}^{\infty}$ be corresponding subsequences of multipliers. First, we show that $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu} (\bm{x}_k,1) \}_{k=0}^{\infty}$ are uniformly bounded for $k$ sufficiently large. Rearranging the terms in equation (\ref{prob:pasa-error}.1) we have that 
\begin{align*}
\begin{bmatrix}
\nabla \bm{h} (\bm{x}_k)^{\intercal} \ \vert \ \nabla \bm{r} (\bm{x}_k)^{\intercal}
\end{bmatrix} \begin{bmatrix}
\bm{\lambda}_k \\
\bm{\mu} (\bm{x}_k)
\end{bmatrix}
= \bm{x}_k - \bm{y}(\bm{x}_k) - \nabla f (\bm{x}_k)^{\intercal}
\end{align*}
By our hypothesis that $\nabla \bm{h} (\bm{x}^*)$ and $\nabla \bm{r} (\bm{x}^*)$ are of full rank, there exists a $N$ such that the matrix $\begin{bmatrix} \nabla \bm{h} (\bm{x}_k)^{\intercal} \ \vert \ \bm{r} (\bm{x}_k)^{\intercal} \end{bmatrix}$ is of full rank, for all $k \geq N$. Hence, there exists a constant $M$ such that
\begin{align}
\left\| \begin{bmatrix}
\bm{\lambda}_k \\
\bm{\mu} (\bm{x}_k)
\end{bmatrix} \right\|
\leq M \| \bm{x}_k - \bm{y}(\bm{x}_k) - \nabla f (\bm{x}_k)^{\intercal} \| 
\leq M ( \eta + \| \nabla f (\bm{x}_k) \|), \label{eq:phase-one-convergence.1}
\end{align}
for $k$ sufficiently large, where the final inequality follows from the triangle inequality together with $\sup_{k \geq 0} E_{\scaleto{PASA}{4pt}} (\bm{x}_k) \leq \eta$. As $f \in \mathcal{C}^1$ it follows from (\ref{eq:phase-one-convergence.1}) that the sequences $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu}(\bm{x}_k) \}_{k=0}^{\infty}$ are uniformly bounded for $k$ sufficiently large. As the sequence $\{ \bm{\bar{\lambda}}_k \}_{k=0}^{\infty}$ is uniformly bounded by construction, there exists a constant $\alpha$ such that $\| \bm{\lambda}_{k} - \bm{\bar{\lambda}}_{k-1} \| \leq \alpha$ for all $k$ sufficiently large. Now using the update formula $\bm{\lambda}_{k} = \bm{\bar{\lambda}}_{k-1} + 2 q_k \bm{h} (\bm{x}_{k})$, we have that
\begin{align*}
\bm{h} (\bm{x}_{k}) = \frac{\bm{\lambda}_{k} - \bm{\bar{\lambda}}_{k-1}}{2 q_k}.
\end{align*}
which, together with the hypothesis that $q_k \to \infty$ as $k \to \infty$, yields that
\begin{align*}
\lim_{k \to \infty} E_c (\bm{x}_{k}) = \lim_{k \to \infty} \| \bm{h} (\bm{x}_{k}) \|^2 \leq \lim_{k \to \infty} \frac{\alpha^2}{2 q_k} = 0.
\end{align*}
Finally, as $E_0 (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k))^2 = E_m (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k)) + E_c (\bm{x}_k)$ and $E_m (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k)) \leq \theta E_c (\bm{x}_k)$ for all $k$ by hypothesis, it now follows that $E_0 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu} (\bm{x}^*)) = 0$.
\end{proof}
\fi
%

Our next discussion in this section focuses on establishing a global convergence result for the augmented Lagrangian problem like Theorem~\ref{thm:pasa-aug-lag} but that does not require assumption (\ref{result:pasa-aug-lag-conv.1}). To this end, we propose a slight modification to the PASA algorithm, Algorithm 2 in \cite{Hager2016}, that requires replacing all instances of $E_{\scaleto{PASA}{4pt}} (\bm{x})$ with $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu}(\bm{x},1)) = -\nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},1) - \bm{x})$. This modification is provided in detail in Algorithm~\ref{alg:pasa-aug-lag}. First, we provide a necessary lemma that considers the relationship of the multiplier error estimator $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\alpha)/\alpha)$ to $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\beta)/\beta)$ for various values of $0 < \alpha \leq \beta$. 
\begin{lemma} \label{thm:aug-lag-mult-error}
For a given $\bm{x}$, let $\bm{\mu} (\bm{x}, \alpha)$ satisfy the KKT conditions in (\ref{prob:pasa-error}.1) -- (\ref{prob:pasa-error}.4). Then
\iffalse
\begin{enumerate}
\item[(\ref{thm:aug-lag-mult-error}.1)] For $0 < \alpha \leq \beta$, $-\nabla \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},\alpha) - \bm{x}) 
\leq -\nabla_x \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},\beta) - \bm{x})$. \vspace{1mm}
%%%%%%%%%%%%%%%% NOT NEEDED FOR PAPER %%%%%%%%%%%%%%%%%%%%%%
\iffalse 
\item[(\ref{thm:aug-lag-mult-error}.2old)] For $0 < \alpha \leq \beta$, $- \alpha \nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},\beta) - \bm{x}) 
\leq - \beta \nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},\alpha) - \bm{x})$. \vspace{1mm}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item[(\ref{thm:aug-lag-mult-error}.2)] If $0 < \alpha \leq \beta \leq 1$ then $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\beta)/\beta) 
\leq E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\alpha)/\alpha)$. 
%%%%%%%%%%%%%%%% NOT NEEDED FOR PAPER %%%%%%%%%%%%%%%%%%%%%%
\iffalse 
\vspace{1mm}
\item[(\ref{thm:aug-lag-mult-error}.4)] If $1 \leq \alpha \leq \beta \leq 3$ then
\begin{align*}
\alpha E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\beta)/\beta) 
\leq \beta E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\alpha)/\alpha).
\end{align*}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{enumerate}
\fi
\begin{align}
&-\nabla \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},\alpha) - \bm{x}) 
\leq -\nabla_x \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},\beta) - \bm{x}), \ \text{for} \ 0 < \alpha \leq \beta, \label{thm:aug-lag-mult-error.1} \\
&E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\beta)/\beta) 
\leq E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\alpha)/\alpha), \ \text{for} \ 0 < \alpha \leq \beta \leq 1. \label{thm:aug-lag-mult-error.2}
\end{align}
\end{lemma}
\begin{proof}
Suppose $0 < \alpha \leq \beta$. Let $\bm{d}^{\alpha} (\bm{x}) = \bm{y} (\bm{x}, \alpha) - \bm{x}$. By P1 in \cite{Hager2006} with $\bm{x} \gets \bm{x} - \alpha \bm{g} (\bm{x})$ and $\bm{y} \gets \bm{y} (\bm{x}, \beta)$, we have that
\begin{align}
0 
&\leq (\bm{y} (\bm{x}, \alpha) - (\bm{x} - \alpha \bm{g} (\bm{x})))^{\intercal} (\bm{y} (\bm{x}, \beta) - \bm{y} (\bm{x},\alpha)) \\
&= ( \bm{d}^{\alpha} (\bm{x}) + \alpha \bm{g} (\bm{x}))^{\intercal} (\bm{d}^{\beta} (\bm{x}) - \bm{d}^{\alpha} (\bm{x})) \\
&= \bm{d}^{\alpha} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) - \| \bm{d}^{\alpha} (\bm{x}) \|^2 + \alpha \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) - \alpha \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}).
\end{align}
Rearranging terms and dividing both sides by $\alpha$ yields
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \frac{1}{\alpha} \bm{d}^{\alpha} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) - \frac{1}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|^2.
\end{align}
It now follows from Cauchy-Schwarz that
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \frac{1}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \| \| \bm{d}^{\beta} (\bm{x}) \| - \frac{1}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|^2. \label{eq:aug-lag-mult-error.1}
\end{align}
By swapping $\alpha$ and $\beta$ in the construction of (\ref{eq:aug-lag-mult-error.1}), we obtain the inequality
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) + \frac{1}{\beta} \| \bm{d}^{\beta} (\bm{x}) \| \| \bm{d}^{\alpha} (\bm{x}) \| - \frac{1}{\beta} \| \bm{d}^{\beta} (\bm{x}) \|^2. \label{eq:aug-lag-mult-error.1.1}
\end{align}

As $\alpha \leq \beta$, by P4 in \cite{Hager2006} we have that $\| \bm{d}^{\alpha} (\bm{x}) \| \leq \| \bm{d}^{\beta} (\bm{x}) \|$. Substituting this into (\ref{eq:aug-lag-mult-error.1.1}) yields
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) + \frac{1}{\beta} \| \bm{d}^{\beta} (\bm{x}) \|^2 - \frac{1}{\beta} \| \bm{d}^{\beta} (\bm{x}) \|^2 
= - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}). \label{eq:aug-lag-mult-error.2.1}
\end{align}
which is equivalent to (\ref{thm:aug-lag-mult-error.1}). 

%%%%%%%%%%%%%%%% NOT NEEDED FOR PAPER %%%%%%%%%%%%%%%%%%%%%%
\iffalse 
By P5 in \cite{Hager2006}, we have that $\| \bm{d}^{\beta} (\bm{x}) \| \leq \frac{\beta}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|$ which combined with (\ref{eq:aug-lag-mult-error.1}) yields
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \frac{\beta}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2 - \frac{1}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|^2 \nonumber \\
&= - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \left( \frac{\beta - \alpha}{\alpha} \right) \frac{\| \bm{d}^{\alpha} (\bm{x}) \|^2}{\alpha}. \label{eq:aug-lag-mult-error.2.2}
\end{align}
By P6 in \cite{Hager2006} and the fact that $\beta - \alpha \geq 0$, we have that
\begin{align}
\left( \frac{\beta - \alpha}{\alpha} \right) \frac{\| \bm{d}^{\alpha} (\bm{x}) \|^2}{\alpha}
\leq \left( \frac{\beta - \alpha}{\alpha} \right) \left( - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) \right)
= \left( 1 - \frac{\beta}{\alpha} \right) \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}). \label{eq:aug-lag-mult-error.2.3}
\end{align}
Now (\ref{eq:aug-lag-mult-error.2.2}) and (\ref{eq:aug-lag-mult-error.2.3}) yield
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) 
&\leq - \frac{\beta}{\alpha}  \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) \label{eq:aug-lag-mult-error.2.4}
\end{align}
which is equivalent to (\ref{thm:aug-lag-mult-error}.2old).
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Now suppose that $\alpha \leq \beta \leq 1$. By P5 in \cite{Hager2006}, we have that $\| \bm{d}^{\beta} (\bm{x}) \| \leq \frac{\beta}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|$. Substituting this into (\ref{eq:aug-lag-mult-error.1}) yields
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \frac{\beta}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2 - \frac{1}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|^2 \\
&= - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \left( \frac{1}{\alpha^2} - \frac{1}{\alpha} \right) \| \bm{d}^{\alpha} (\bm{x}) \|^2 - \frac{1 - \beta}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2. \label{eq:aug-lag-mult-error.3}
\end{align}
Again, by P5 in \cite{Hager2006} we have that $-\frac{1}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2 \leq - \frac{1}{\beta^2} \| \bm{d}^{\beta} (\bm{x}) \|$ and since $1 - \beta \geq 0$ it follows that 
\begin{align}
- \frac{1 - \beta}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2 
\leq - \frac{1 - \beta}{\beta^2} \| \bm{d}^{\beta} (\bm{x}) \|^2
= - \left( \frac{1}{\beta^2} - \frac{1}{\beta} \right) \| \bm{d}^{\beta} (\bm{x}) \|^2. \label{eq:aug-lag-mult-error.3.1}
\end{align}
Combining (\ref{eq:aug-lag-mult-error.3}) and (\ref{eq:aug-lag-mult-error.3.1}) and rearranging terms yields
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) + \left( \frac{1}{\beta^2} - \frac{1}{\beta} \right) \| \bm{d}^{\beta} (\bm{x}) \|^2
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \left( \frac{1}{\alpha^2} - \frac{1}{\alpha} \right) \| \bm{d}^{\alpha} (\bm{x}) \|^2 \label{eq:aug-lag-mult-error.3.2}
\end{align}
which by (\ref{eq:aug-lag-mod.4}) is equivalent to (\ref{thm:aug-lag-mult-error.2}).
%%%%%%%%%%%%%%%% NOT NEEDED FOR PAPER %%%%%%%%%%%%%%%%%%%%%%
\iffalse 
Now suppose that $1 \leq \alpha \leq \beta \leq 3$. By P5 in \cite{Hager2006}, we have that $-\frac{1}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2 \leq - \frac{1}{\beta^2} \| \bm{d}^{\beta} (\bm{x}) \|$. Combining this with $\frac{1 - \beta}{\beta^3} \leq \frac{1 - \alpha}{\alpha^3} \leq 0$ for $1 \leq \alpha \leq \beta \leq 3$ yields
\begin{align}
\alpha \left(\frac{1 - \beta}{\beta^2} \right) \| \bm{d}^{\beta} (\bm{x}) \|^2 
\leq \beta \left( \frac{1 - \alpha}{\alpha^2} \right) \| \bm{d}^{\alpha} (\bm{x}) \|^2.
\label{eq:aug-lag-mult-error.4}
\end{align}
As $\alpha \leq \beta$, combining (\ref{thm:aug-lag-mult-error.2}) with (\ref{eq:aug-lag-mult-error.4}) it follows that
\begin{align}
- \alpha \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) + \alpha \left( \frac{1}{\beta^2} - \frac{1}{\beta} \right) \| \bm{d}^{\beta} (\bm{x}) \|^2
&\leq - \beta \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \beta \left( \frac{1}{\alpha^2} - \frac{1}{\alpha} \right) \| \bm{d}^{\alpha} (\bm{x}) \|^2 \label{eq:aug-lag-mult-error.4.1}
\end{align}
By the formula for $E_{m,0}$ in (\ref{eq:aug-lag-mod.4}), we have
\begin{align}
\alpha E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\beta)/\beta) 
\leq \beta E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\alpha)/\alpha) \label{eq:aug-lag-mult-error.4.2}
\end{align}
which shows that (\ref{thm:aug-lag-mult-error}.4) holds.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{proof}

With this lemma established, we now provide the following convergence result for the gradient projection algorithm in phase one of PASA. This result is similar to Theorem 2.2 in \cite{Hager2006}.

\begin{theorem} \label{thm:ngpa-conv}
Given $\bm{u}_0 \in \mathbb{R}^n$, $\bm{\bar{\lambda}}_k$, and $q_k$ suppose that (G1) and (G2) hold at $(\bm{u}_0, \bm{\bar{\lambda}}_k, q_k)$. If the nonmonotone gradient projection algorithm (NGPA) in \cite{Hager2006} with $\varepsilon = 0$ is used to solve problem (\ref{prob:aug-lag-mod}) then NGPA either terminates in a finite number of iterations at a stationary point, or generates a sequence of iterates $\{ \bm{u}_i \}_{i=0}^{\infty}$ satisfying
\begin{align}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) = 0.
\end{align}
\end{theorem}
\begin{proof}
Let $F(\bm{x}) = \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k)$. First, note that from (3.6) in \cite{Hager2016}, the stepsize $s_k$ in the Armijo line search is bounded below by
\begin{align}
s_k \geq \min \left\{ 1, \frac{2 \eta (1 - \delta)}{\kappa \alpha_{\max}} \right\} =: c,
\end{align}
where $\kappa$ is the Lipschitz constant for $\nabla_x \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k)$. From equation (2.16) in \cite{Hager2006} we have that
\begin{align}
- \delta c \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i) \leq F_i^r - F (\bm{u}_{i+1}), \label{eq:gpa-conv.1}
\end{align}
for some $\bar{\alpha}_i \in [\alpha_{\min}, \alpha_{\max}]$. We now proceed by way of contradiction. Accordingly, suppose that 
\begin{align}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) > 0.
\end{align}
Then there exists a constant $\tau > 0$ such that 
\begin{align}
\tau \leq E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) 
= - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, 1) - \bm{u}_i), \label{eq:gpa-conv.2}
\end{align}
for all $i \geq 0$. Suppose $\bar{\alpha}_i \geq 1$. By (\ref{thm:aug-lag-mult-error.1}) in Theorem~\ref{thm:aug-lag-mult-error} with $\alpha = 1$ and $\beta = \bar{\alpha}_i$, we have
\begin{align}
\tau \leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, 1) - \bm{u}_i) 
\leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i). \label{eq:gpa-conv.3}
\end{align}
On the other hand, if $\bar{\alpha}_i \in (0,1)$ then by (\ref{thm:aug-lag-mult-error.2}) in Theorem~\ref{thm:aug-lag-mult-error} with $\alpha = \bar{\alpha}_i$ and $\beta = 1$ we have
\begin{align}
- \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, 1) - \bm{u}_i) 
\leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i) + \left( \frac{1}{\bar{\alpha}_i} - 1 \right) \frac{\| \bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i \|^2}{\bar{\alpha}_i}. \label{eq:gpa-conv.4}
\end{align}
From P6 in \cite{Hager2006} we have that 
\begin{align}
\frac{\| \bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i \|^2}{\bar{\alpha}_i} \leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i). \label{eq:gpa-conv.5}
\end{align}
As $\bar{\alpha}_i \in (0,1)$, we have that $\left( \frac{1}{\bar{\alpha}_i} - 1 \right) > 0$ which combined with (\ref{eq:gpa-conv.5}) yields
\begin{align}
\left( \frac{1}{\bar{\alpha}_i} - 1 \right) \frac{\| \bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i \|^2}{\bar{\alpha}_i} 
&\leq \left( \frac{1}{\bar{\alpha}_i} - 1 \right) \left( - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) \right) %\nonumber \\
= \left( 1 - \frac{1}{\bar{\alpha}_i} \right) \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i). \label{eq:gpa-conv.6}
\end{align}
From (\ref{eq:gpa-conv.4}) and (\ref{eq:gpa-conv.6}) it now follows that
\begin{align}
- \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, 1) - \bm{u}_i) \leq - \frac{1}{\bar{\alpha}_i} \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i). \label{eq:gpa-conv.7}
\end{align}
As $\bar{\alpha}_i \geq \alpha_{\min}$, (\ref{eq:gpa-conv.2}) and (\ref{eq:gpa-conv.7}) now yield
\begin{align}
\alpha_{\min} \tau \leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i). \label{eq:gpa-conv.8}
\end{align}
Hence, by observing (\ref{eq:gpa-conv.3}) and (\ref{eq:gpa-conv.8}) we have established that for any choice of $\bar{\alpha}_i \in [\alpha_{\min}, \alpha_{\max}]$ there exists a constant $\nu$ such that
\begin{align}
\nu \leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i). \label{eq:gpa-conv.9}
\end{align}
Combining (\ref{eq:gpa-conv.1}) and (\ref{eq:gpa-conv.9}) yields
\begin{align}
F (\bm{u}_{i+1}) \leq F_i^r - \delta c \nu \label{eq:gpa-conv.10}
\end{align}
which, by the same argument in the proof of Theorem 2.2 of \cite{Hager2006}, results in a contradiction. Thus, we have
\begin{align}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) = 0,
\end{align}
which concludes the proof.
\end{proof}

With this convergence theorem established for the nonmonotone gradient projection algorithm (NGPA) in \cite{Hager2006}, we now provide Algorithm~\ref{alg:pasa-aug-lag} which is PASA with modified stopping and branching criterion designed for the augmented Lagrangian problem (\ref{prob:aug-lag-mod}). The only change here is that we have modified the stopping criterion. Traditionally, the stopping criterion in PASA at the iterate $\bm{x}$ is given by $E_{\scaleto{PASA}{4pt}} (\bm{x}) \leq \varepsilon$, where $\varepsilon$ is a user provided stopping tolerance value. We have modified this criterion by replacing $E_{\scaleto{PASA}{4pt}}$ with $E_{m,0}$ and intend to use the formula in (\ref{eq:aug-lag-mod.4}) to compute $E_{m,0}$.
\begin{center}
\begin{algorithm}
%	\algsetup{linenosize=\notsotiny}
%	\notsotiny
	\caption{Modified PASA Algorithm for GS Augmented Lagrangian Problem} \label{alg:pasa-aug-lag} 
    % Initialize parameters
	{\bfseries Inputs:} Initial guess $\bm{x}_k$, scalar parameters $\theta \in (0,1)$, $\gamma \in (0,1)$, $\varepsilon > 0$, $q_k > 0$ and vector parameter $\bm{\bar{\lambda}}_k$\\
	Set $\bm{u}_{0} = \bm{x}_{k}$, $\bm{u}_1 = \mathcal{P}_{\Omega} (\bm{u}_0)$, and $i = 1$\\
    % Phase one
	\textbf{Phase one}:\\
    \While{$E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) > \varepsilon$}{
        Set $\bm{u}_{i+1} \gets GPA(\bm{u}_i)$ and $i \gets i+1$\\
        \If{$\mathcal{U} (\bm{u}_i) = \emptyset$ \textbf{and} $e_{\scaleto{PASA}{4pt}} (\bm{u}_i) < \theta E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1))$}{
            Set $\theta \gets \gamma \theta$
        }
        \If{$e_{\scaleto{PASA}{4pt}} (\bm{u}_i) \geq \theta E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1))$}{
    	    \textbf{goto} phase two
        }
    }
    % Phase two 
	\textbf{Phase two}:\\ 
    \While{$E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) > \varepsilon$}{
        Set $\bm{u}_{i+1} \gets LCO(\bm{u}_i)$ and $i \gets i+1$\\
        \If{$e_{\scaleto{PASA}{4pt}} (\bm{u}_i) < \theta E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1))$}{
       	    \textbf{goto} phase one
        }
    }
    \textbf{Return} $\bm{u}_i$
\end{algorithm}
\end{center}
As some justification for this modification, in (\ref{eq:aug-lag-mod.5}) we establish that $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) \leq \| \nabla \mathcal{L} (\bm{x}, \bm{\bar{\lambda}}_k) \| E_{\scaleto{PASA}{4pt}} (\bm{x})$. So if PASA terminates using its regular stopping criterion at a point $\bm{x}$ where $\| \nabla \mathcal{L} (\bm{x}, \bm{\bar{\lambda}}_k) \| > 1$ then it is possible that $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) > \varepsilon$. %Note that both of the vectors required for the dot product are already available at each iteration of PASA due to the use of the gradient of the cost function and the need to check the regular stopping criterion for PASA. 
Alternatively, to ensure that the branching criterion between for phase one to phase two NPASA is satisfied, we could instead terminate when 
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) 
= - \nabla_x \mathcal{L}_{q_k} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y}(\bm{x},1) - \bm{x}) 
\leq \min \left\{ \varepsilon, \theta E_c (\bm{x}) \right\}. \label{eq:pasa-aug-lag-stop-crit2}
\end{align}
%In addition to an evaluation of the dot product for the left hand side of the inequality, this would require an evaluation of the equality constraints for the right hand side. However, as updating the multipliers $\bm{\bar{\lambda}}_k$ requires evaluating the equality constraints then we can compute the norm after evaluating these constraints to check the branching criterion. Note that if the hypotheses of Theorem~\ref{thm:pasa-aug-lag-conv} hold then the new stopping criterion in (\ref{eq:pasa-aug-lag-stop-crit1}) will be satisfied for any augmented Lagrangian problem in which the original stopping criterion, $E_{\scaleto{PASA}{4pt}}(\bm{x}) \leq \varepsilon$, will be satisfied.

We now consider a global convergence result for Algorithm~\ref{alg:pasa-aug-lag} which is similar to Theorem 3.2 in \cite{Hager2016}. The benefit to using Algorithm~\ref{alg:pasa-aug-lag} to solve problem (\ref{prob:aug-lag-mod}) instead of the original version of PASA in \cite{Hager2016} is that when using Algorithm~\ref{alg:pasa-aug-lag} we no longer require the additional assumption that the sequence $\{ \bm{u}_i \}_{i=1}^{\infty}$ generated by PASA satisfies (\ref{result:pasa-aug-lag-conv.1}) that was required in Theorem~\ref{thm:pasa-aug-lag} to establish global convergence for the multiplier error.

\begin{theorem} \label{thm:pasa-aug-lag-mod-global-conv}
Given $\bm{u}_0 \in \mathbb{R}^n$, $\bm{\bar{\lambda}}_k$, and $q_k$ suppose that (G1) and (G2) hold at $(\bm{u}_0, \bm{\bar{\lambda}}_k, q_k)$. If Algorithm~\ref{alg:pasa-aug-lag} with $\varepsilon = 0$ is used to solve problem (\ref{prob:aug-lag-mod}) then Algorithm~\ref{alg:pasa-aug-lag} either terminates in a finite number of iterations at a stationary point, or generates a sequence of iterates $\{ \bm{u}_i \}_{i=0}^{\infty}$ satisfying
\begin{align}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) = 0. \label{result:pasa-aug-lag-mod-global-conv}
\end{align}
\end{theorem}
\begin{proof}
The proof is split into three cases.\\
{\bfseries Case 1: Phase two of Algorithm~\ref{alg:pasa-aug-lag} is executed a finite number of times.} In this case, only phase one of Algorithm~\ref{alg:pasa-aug-lag} is executed for $i$ sufficiently large. As such, from Theorem~\ref{thm:ngpa-conv} it follows that (\ref{result:pasa-aug-lag-mod-global-conv}) holds. \\
{\bfseries Case 2: Phase one of Algorithm~\ref{alg:pasa-aug-lag} is executed a finite number of times.} Here, only phase two is executed for $i$ sufficiently large. Since phase two eventually does not branch back to phase one, by the branching criterion in phase two we have that
\begin{align}
\theta E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) \leq e_{\scaleto{PASA}{4pt}} (\bm{u}_i)
\end{align}
for $i$ sufficiently large. Using an argument found in the proof of Theorem 3.2 from \cite{Hager2016} we have that (\ref{result:pasa-aug-lag-mod-global-conv}) holds. \\
{\bfseries Case 3: Phases one and two of Algorithm~\ref{alg:pasa-aug-lag} are executed an infinite number of times.} By way of contradiction, assume that (\ref{result:pasa-aug-lag-mod-global-conv}) does not hold. Then there exists a constant $\tau > 0$ such that 
\begin{align}
\tau \leq E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q_k \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) = - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, 1) - \bm{u}_i).
\end{align}
Letting $F (\bm{u}_{i+1}) = \mathcal{L}_{q_k} (\bm{u}_{i+1}, \bm{\bar{\lambda}}_k)$ and applying the same argument as in the proof of Theorem~\ref{thm:ngpa-conv}, we have that there exists a constant $\nu$ such that
\begin{align}
F (\bm{u}_{i+1}) \leq F (\bm{u}_i) - \delta c \nu \label{eq:pasa-aug-lag-mod-global-conv.10}
\end{align}
for each iteration of GPA when $i$ is sufficiently large. Additionally, by property F1 of the LCO in \cite{Hager2016}, we have that $F (\bm{u}_{i+1}) \leq F (\bm{u}_i)$. Since there are an infinite number of iterations in phase one, it follows that the cost function is unbounded from below which contradictions assumption (G1). Thus, (\ref{result:pasa-aug-lag-mod-global-conv}) holds.
\end{proof}

Based on the analysis in this section, we note that Algorithm~\ref{alg:pasa-aug-lag} should be used to solve the augmented Lagrangian problem in the GS algorithm in phase one of NPASA. As we were able to establish a global convergence result for the multiplier error of the original nonlinear program with the same set of assumptions required for global convergence of the PASA error estimator, Algorithm~\ref{alg:pasa-aug-lag} is more suitable for problem (\ref{prob:aug-lag-mod}) than the original version of PASA for solving the nonlinear program.

At this point, we have addressed nearly every step of phase one of NPASA. However, throughout the analysis in this section we have treated $\bm{\mu} (\bm{x}_k, 1)$ as a vector that exists but that is not explicitly known. While the formula for $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1))$ provided in (\ref{eq:aug-lag-mod.4.2}) proved useful in establishing convergence of the augmented Lagrangian problem phase one of NPASA and allows the user to compute an error estimator without requiring the value of $\bm{\mu} (\bm{x}_k,1)$, to establish desirable global convergence properties for NPASA in Section~\ref{section:npasa-global-convergence} we need to compute $E_{m,1} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1))$ at the end of phase one of NPASA. As the vector $\bm{\mu} (\bm{x}_k, 1)$ is required to compute $E_1 (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k, 1))$, we now discuss how to construct the vector $\bm{\mu} (\bm{x}_k, 1)$ using information already computed internally by PASA when solving the augmented Lagrangian problem in (\ref{prob:aug-lag-mod}). When checking the stopping criterion for the original PASA algorithm \cite{HagerActive} or for the modified PASA algorithm presented here in Algorithm~\ref{alg:pasa-aug-lag}, it is necessary to solve problem (\ref{prob:pasa-error}) with $\alpha = 1$, restated here as
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{y}} & \frac{1}{2} \| \bm{x} - \bm{g} (\bm{x}) - \bm{y} \|^2 \\
\text{s.t.} & \bm{y} \in \Omega.
\end{array} \label{prob:pasa-construct-mult}
\end{align}
where $\bm{x}$ is fixed and we let $\Omega$ be of the general form $\Omega = \{ \bm{y} : \bm{\ell} \leq \bm{A} \bm{y} \leq \bm{u}, \bm{lo} \leq \bm{y} \leq \bm{hi} \}$. In implementation, this problem is solved using a dual technique with the algorithm PPROJ \cite{Hager2016}. From equation (1.5) in \cite{Hager2016} PPROJ computes a solution for the dual variable, which we will denote by $\bm{\pi}^*$, that is used to reconstruct the primal solution, $\bm{y} (\bm{\pi}^*)$. Letting $\bm{a}_i$ denote the $i$th column of $\bm{A}$ and $\bm{a}_j^{\intercal}$ denote the $j$th row of $A$, using equation (1.5) in \cite{Hager2016} we have that this primal solution satisfies
\begin{align}
y_i (\bm{\pi}^*) = \left\{
	\begin{array}{lll}
	lo_i & : & x_i - g_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^* \leq lo_i \vspace{0.8mm} \\
	hi_i & : & x_i - g_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^* \geq hi_i \vspace{0.8mm} \\
    x_i - g_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^* & : & \text{otherwise}
	\end{array}
	\right. \label{eq:pasa-construct-mult.1}
\end{align}
and
\begin{align}
\bm{a}_j^{\intercal} \bm{y} (\bm{\pi}^*) = \left\{
	\begin{array}{lll}
	\ell_j & : & \pi_j^* > 0 \\
	u_j & : & \pi_j^* < 0
	\end{array}
	\right., \label{eq:pasa-construct-mult.2}
\end{align}
for $1 \leq i \leq n$ and $1 \leq j \leq m$. Now consider the Lagangian for problem (\ref{prob:pasa-construct-mult}) given by
\begin{align}
L (\bm{y}, \bm{\gamma}_1, \bm{\gamma}_2, \bm{\upsilon}_1, \bm{\upsilon}_2) 
&= \frac{1}{2} \| \bm{x} - \bm{g} (\bm{x}) - \bm{y} \|^2 + \bm{\gamma}_1^{\intercal} (\bm{\ell} - \bm{A} \bm{y}) + \bm{\gamma}_2^{\intercal} (\bm{A} \bm{y} - \bm{u}) \nonumber \\
&\quad + \bm{\upsilon}_1^{\intercal} (\bm{lo} - \bm{y}) + \bm{\upsilon}_2^{\intercal} ( \bm{y} - \bm{hi}). \label{eq:pasa-construct-mult.3}
\end{align}
It follows that
\begin{align}
\nabla_y L (\bm{y}, \bm{\gamma}_1, \bm{\gamma}_2, \bm{\upsilon}_1, \bm{\upsilon}_2)^{\intercal} 
&= \bm{y} - (\bm{x} - \bm{g} (\bm{x}))  - \bm{A}^{\intercal} \bm{\gamma}_1 + \bm{A}^{\intercal} \bm{\gamma}_2 - \bm{\upsilon}_1 + \bm{\upsilon}_2. \label{eq:pasa-construct-mult.4}
\end{align}
%Letting $\bm{y}^* = \bm{y} (\bm{\pi}^*)$, we proceed by partitioning $\bm{y}^*$ into three parts, denoted $\bm{y}_{\mathcal{S}_1}^*$, $\bm{y}_{\mathcal{S}_2}^*$, and $\bm{y}_{\mathcal{S}_3}^*$, where the index sets used to construct the partition of $\bm{y}^*$ are defined by $\mathcal{S}_1 = \{ i \in \mathbb{N} : \bm{y}_i^* = lo_i \}$, $\mathcal{S}_2 = \{ i \in \mathbb{N} : \bm{y}_i^* = hi_i \}$, and $\mathcal{S}_3 = \{ i \in \mathbb{N} : lo_i < \bm{y}_i^* < hi_i \}$. 
Now let $\bm{y}^* = \bm{y} (\bm{\pi}^*)$ and define the index sets $\mathcal{S}_1 = \{ i \in \mathbb{N} : \bm{y}_i^* = lo_i \}$, $\mathcal{S}_2 = \{ i \in \mathbb{N} : \bm{y}_i^* = hi_i \}$, and $\mathcal{S}_3 = \{ i \in \mathbb{N} : lo_i < \bm{y}_i^* < hi_i \}$. Using $\bm{y}^*$, $\bm{\pi}^*$, and the sets $\mathcal{S}_j$, for $j \in \{ 1, 2, 3 \}$, we work to construct multiplier vectors $\bm{\gamma}_1^*$, $\bm{\gamma}_2^*$, $\bm{\upsilon}_1^*$, and $\bm{\upsilon}_2^*$ that satisfy the KKT conditions for problem (\ref{prob:pasa-construct-mult}) given by:
\begin{enumerate}
\item[(M.1)] Gradient of Lagrangian equals zero: $\nabla_y L (\bm{y}^*, \bm{\gamma}_1^*, \bm{\gamma}_2^*, \bm{\upsilon}_1^*, \bm{\upsilon}_2^*)^{\intercal} = \bm{0}$
\item[(M.2)] Satisfies problem constraints: $\bm{y}^* \in \Omega$
\item[(M.3)] Nonnegativity of inequality multipliers: $\bm{\gamma}_1^*, \bm{\gamma}_2^* \in \mathbb{R}_{\geq 0}^{m}$ and $\bm{\upsilon}_1^*, \bm{\upsilon}_2^* \in \mathbb{R}_{\geq 0}^{n}$
\item[(M.4)] Complimentary slackness: $(\bm{\ell} - \bm{A} \bm{y}^*)^{\intercal} \bm{\gamma}_1^* = 0$, $(\bm{A} \bm{y}^* - \bm{u})^{\intercal} \bm{\gamma}_2^* = 0$, $(\bm{lo} - \bm{y}^*)^{\intercal} \bm{\upsilon}_1^* = 0$, and $(\bm{y}^* - \bm{hi})^{\intercal} \bm{\upsilon}_2^* = 0$.
\end{enumerate}
Note that (M.2) is already satisfied. First, we define the components of vectors $\bm{\gamma}_1^*$ and $\bm{\gamma}_2^*$ by
\begin{align}
\gamma_{1,j}^* := \left\{
	\begin{array}{cll}
	\pi_j^* & : & \pi_j^* > 0 \\
	0 & : & \text{otherwise}
	\end{array}
	\right. \label{eq:pasa-construct-mult.5}
\end{align}
and
\begin{align}
\gamma_{2,j}^* := \left\{
	\begin{array}{cll}
	-\pi_j^* & : & \pi_j^* < 0 \\
	0 & : & \text{otherwise}
	\end{array}
	\right., \label{eq:pasa-construct-mult.6}
\end{align}
respectively, for $1 \leq j \leq m$. By definition, we have that $\bm{\gamma}_1^*, \bm{\gamma}_2^* \in \mathbb{R}_{\geq 0}^{m}$. Also, it follows from definition that
\begin{align}
\bm{\gamma}_1^* - \bm{\gamma}_2^* 
= \bm{\pi}^*. \label{eq:pasa-construct-mult.6.1}
\end{align}
Additionally, combining (\ref{eq:pasa-construct-mult.2}), (\ref{eq:pasa-construct-mult.5}), and (\ref{eq:pasa-construct-mult.6}) it follows that $(\bm{\ell} - \bm{A} \bm{y}^*)^{\intercal} \bm{\gamma}_1^* = 0$ and $(\bm{A} \bm{y}^* - \bm{u})^{\intercal} \bm{\gamma}_2^* = 0$. Next, we define vectors $\bm{\upsilon}_1^*$ and $\bm{\upsilon}_2^*$ componentwise by
\begin{align}
\upsilon_{1,i}^* := \left\{
	\begin{array}{lll}
	lo_i - (x_i - \bm{g}_i (\bm{x})) - \bm{a}_i^{\intercal} \bm{\pi}^* & : & i \in \mathcal{S}_1 \\
	0 & : & i \in \mathcal{S}_2 \cup \mathcal{S}_3
	\end{array}
	\right. \label{eq:pasa-construct-mult.7}
\end{align}
and
\begin{align}
\upsilon_{2,i}^* := \left\{
	\begin{array}{lll}
	-hi_i + x_i - \bm{g}_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^* & : & i \in \mathcal{S}_2 \\
	0 & : & i \in \mathcal{S}_1 \cup \mathcal{S}_3
	\end{array}
	\right., \label{eq:pasa-construct-mult.8}
\end{align}
respectively. By the definition of $\mathcal{S}_1$ and (\ref{eq:pasa-construct-mult.1}), we have that
\begin{align}
lo_i - (x_i - \bm{g}_i (\bm{x})) - \bm{a}_i^{\intercal} \bm{\pi}^* \geq 0, \quad \text{for all $i \in \mathcal{S}_1$.} \label{eq:pasa-construct-mult.9}
\end{align}
As $\upsilon_{1,i}^* = 0$ for $i \in \mathcal{S}_2 \cup \mathcal{S}_3$ it now follows that $\bm{\upsilon}_1^* \in \mathbb{R}_{\geq 0}^{n}$. Similarly, by the definition of $\mathcal{S}_2$ and (\ref{eq:pasa-construct-mult.1}) it follows that
\begin{align}
-hi_i + (x_i - \bm{g}_i (\bm{x})) + \bm{a}_i^{\intercal} \bm{\pi}^* \geq 0, \quad \text{for all $i \in \mathcal{S}_2$.} \label{eq:pasa-construct-mult.10}
\end{align}
As $\upsilon_{2,i}^* = 0$ for $i \in \mathcal{S}_1 \cup \mathcal{S}_3$ it now follows that $\bm{\upsilon}_2^* \in \mathbb{R}_{\geq 0}^{n}$. Hence, (M.3) holds. Next, combining (\ref{eq:pasa-construct-mult.2}), (\ref{eq:pasa-construct-mult.9}), and (\ref{eq:pasa-construct-mult.10}) it follows that $(\bm{lo} - \bm{y}^*)^{\intercal} \bm{\upsilon}_1^* = 0$ and $(\bm{y}^* - \bm{hi})^{\intercal} \bm{\upsilon}_2^* = 0$. Hence, (M.4) holds. Lastly, it remains to show that (M.1) holds. Combining (\ref{eq:pasa-construct-mult.4}) and (\ref{eq:pasa-construct-mult.6.1}) we have that
\begin{align}
\nabla_y L (\bm{y}^*, \bm{\gamma}_1^*, \bm{\gamma}_2^*, \bm{\upsilon}_1^*, \bm{\upsilon}_2^*)^{\intercal} 
&= \bm{y}^* - (\bm{x} - \bm{g} (\bm{x}))  - \bm{A}^{\intercal} \bm{\pi}^* - \bm{\upsilon}_1^* + \bm{\upsilon}_2^*. \label{eq:pasa-construct-mult.11}
\end{align}
To show that (M.1) holds, we need to show that
\begin{align}
\bm{y}_i^* - (x_i - \bm{g}_i (\bm{x}))  - \bm{a}_i^{\intercal} \bm{\pi}^* - \upsilon_{1,i}^* + \upsilon_{2,i}^*
&= 0. \label{eq:pasa-construct-mult.12}
\end{align}
for $1 \leq i \leq n$. Accordingly, fix $i \in \{1, 2, \ldots, n \}$. Suppose $i \in \mathcal{S}_1$. Then using (\ref{eq:pasa-construct-mult.1}), (\ref{eq:pasa-construct-mult.9}), and (\ref{eq:pasa-construct-mult.10}) we have that $\bm{y}_i^* = lo_i$, $\upsilon_{1,i}^* = lo_i - (x_i - \bm{g}_i (\bm{x})) - \bm{a}_i^{\intercal} \bm{\pi}^*$, and $\upsilon_{2,i}^* = 0$, respectively. Hence, (\ref{eq:pasa-construct-mult.12}) holds for $i \in \mathcal{S}_1$. Next suppose $i \in \mathcal{S}_2$. Then using (\ref{eq:pasa-construct-mult.1}), (\ref{eq:pasa-construct-mult.9}), and (\ref{eq:pasa-construct-mult.10}) we have that $\bm{y}_i^* = hi_i$, $\upsilon_{1,i}^* = 0$, and $\upsilon_{2,i}^* = -hi_i + x_i - \bm{g}_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^*$, respectively. Hence, (\ref{eq:pasa-construct-mult.12}) holds for $i \in \mathcal{S}_2$. Lastly, suppose $i \in \mathcal{S}_3$. Then using (\ref{eq:pasa-construct-mult.1}), (\ref{eq:pasa-construct-mult.9}), and (\ref{eq:pasa-construct-mult.10}) we have that $\bm{y}_i^* = x_i - \bm{g}_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^*$, $\upsilon_{1,i}^* = 0$, and $\upsilon_{2,i}^* = 0$, respectively. Hence, (\ref{eq:pasa-construct-mult.12}) holds for $i \in \mathcal{S}_3$. As $\mathcal{S}_1 \cup \mathcal{S}_2 \cup \mathcal{S}_3 = \{ 1, 2, \ldots, n \}$, we conclude that (M.1) holds. Thus, $(\bm{y}^*, \bm{\gamma}_1^*, \bm{\gamma}_2^*, \bm{\upsilon}_1^*, \bm{\upsilon}_2^*)$ is a KKT point for problem (\ref{prob:pasa-construct-mult}). As our goal was to construct the inequality multiplier $\bm{\mu} (\bm{x}, 1)$, we now note that $\bm{y}^* = \bm{y} (\bm{x}^*, 1)$. Hence, when the polyhedral constraints for the original problem are in the standard format
\begin{align}
\bm{r} (\bm{x}) = \begin{bmatrix}
\bm{\ell} - \bm{A} \bm{x} \\
\bm{A} \bm{x} - \bm{u} \\
\bm{lo} - \bm{x} \\
\bm{x} - \bm{hi}
\end{bmatrix}
\end{align}
then it follows that we should construct $\bm{\mu} (\bm{x}^*, 1)$ by
\begin{align}
\bm{\mu} (\bm{x}^*, 1) := \begin{bmatrix}
\bm{\gamma}_1^* \\ 
\bm{\gamma}_2^* \\
\bm{\upsilon}_1^* \\
\bm{\upsilon}_2^*
\end{bmatrix}. \label{eq:pasa-construct-mult.13}
\end{align}
As $\bm{y}^*$ and $\bm{\pi}^*$ are available when completing PPROJ, we can always perform this construction. Note that this construction only needs to be performed once after terminating PASA in phase one since we only need $\bm{\mu} (\bm{x}_k, 1)$ to compute $E_1 (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k, 1))$ at the end of phase one. 

With this construction completed, we have addressed all of the necessary steps for implementing phase one of NPASA as outlined in Algorithms~\ref{alg:gs} and \ref{alg:npasa}. We now turn our attention to phase two of NPASA.

